Measuring Societal Biases from Text Corpora with Smoothed First-Order Co-occurrence

Text corpora are widely used resources for measuring societal biases and stereotypes. The common approach to measuring such biases using a corpus is by calculating the similarities between the embedding vector of a word (like nurse) and the vectors of the representative words of the concepts of interest (such as genders). In this study, we show that, depending on what one aims to quantify as bias, this commonly-used approach can introduce non-relevant concepts into bias measurement. We propose an alternative approach to bias measurement utilizing the smoothed first-order co-occurrence relations between the word and the representative concept words, which we derive by reconstructing the co-occurrence estimates inherent in word embedding models. We compare these approaches by conducting several experiments on the scenario of measuring gender bias of occupational words, according to an English Wikipedia corpus. Our experiments show higher correlations of the measured gender bias with the actual gender bias statistics of the U.S. job market - on two collections and with a variety of word embedding models - using the first-order approach in comparison with the vector similarity-based approaches. The first-order approach also suggests a more severe bias towards female in a few specific occupations than the other approaches.

==> bias_quant.tex <==

In Bolukbasi et al.~\cite{bolukbasi2016man}, the degree of gender bias of a word is measured using the following approach:

\begin{equation}
\begin{aligned}
\widehat{\lambda}_{f}(w)=cosine(\vv_{she}, \vv_w) \\
\widehat{\lambda}_{m}(w)=cosine(\vv_{he}, \vv_w)
\end{aligned}
\label{eq:genderbias:lambdahat}
\end{equation}
where $\widehat{\lambda}_{f}$ ($\widehat{\lambda}_{m}$) denotes the degree of bias of a word  $w$ (occupation in our case) to female (male).


As mentioned in introduction, due to the circularity in word embedding, using $\vv_{she}$ and $\vv_{he}$ does not provide a precise quantification of bias, as these vectors also contain concepts related to the occupations. To validate the existence of circularity, we can use the explicit variations of  $\vv_{she}$ and $\vv_{he}$, namely $\ve_{she}$ and $\ve_{he}$ and examine $e_{she:c}$ and $e_{he:c}$, the values regarding each occupation $c$ (as a concept) in the explicit vector representation of `she' and `he', respectively. Among the 343 occupations, we observe 123, and 168 values higher than zero for $\ve_{she}$ and $\ve_{he}$ respectively, indicating significant existence of occupation-related concepts in the gender vectors.

To address the issue raised by circularity, we first select a set of terms, representing gender-specific concepts in language. These terms are shortlisted from the gender-specific list, provided by Bolukbasi et al. after filtering the occupations. The final list contains 32 female-specific terms (e.g. `she', `her', `woman') and 32 equivalent male-specific terms (e.g. `he', `his', `man'), denoted as $\sG_f$ and $\sG_m$, shown in Table~XF, and Table~XM respectively.

\begin{table*}[t]
\begin{center}
\caption{Correlation results of gender bias, calculated by word representations, to the statistics of the portion of women in occupations in U.S. job market, provided by the datasets in WinoBias~\cite{zhao2018gender} and U.S. Census Data~\cite{garg2018word}}
\centering
\begin{tabular}{l l | l | c c | c  c}
 \multicolumn{2}{c|}{\multirow{2}{*}{Representation}} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{WinoBias} & \multicolumn{2}{c}{U.S. Census Data}  \\
 & &  & Spearman & Pearson & Spearman & Pearson \\\hline
\multirow{6}{*}{\rotatebox[origin=c]{-90}{Count-based}} & PMI-SVD & \multirow{3}{*}{NND} & 0.18 & 0.25 & 0.20 & 0.29\\
 & PPMI-SVD & & 0.18 & 0.25 & 0.20 & 0.29\\
 & SPPMI-SVD & & 0.11 & 0.13 & 0.08 & 0.12\\\cdashline{2-7}
 & PMI & \multirow{3}{*}{Co-occur.}& 0.55 & 0.53  & 0.55 & 0.59\\
 & PPMI & & 0.60  & 0.57  & 0.62 & 0.63\\
 & SPPMI  & & 0.45 & 0.47 & 0.48 & 0.46\\\midrule
\multirow{5}{*}{\rotatebox[origin=c]{-90}{Pred.-based}} & \multirow{2}{*}{SG} & Cosine~\cite{bolukbasi2016man} & 0.53 & 0.55 & 0.57 & 0.62\\
 &  & NND~\cite{garg2018word} & 0.54 & 0.54 & 0.57 & 0.61\\\cdashline{2-7}
 & eSG &  \multirow{3}{*}{Co-occur.}  & \textbf{0.68} & \textbf{0.62} & \textbf{0.67} & \textbf{0.72}\\
 & SeSG & & 0.67 & 0.62 & 0.67 & 0.71\\
 & PSeSG & & 0.66 & 0.55 & 0.64 & 0.66\\
\end{tabular}
\label{tbl:genderbias:correlation} 
\end{center}
\end{table*}

Using these lists gender-concepts, we define the new gender factors as the sum of gender-related concepts of the explicit vector of each word, shown as follows:
\begin{equation}
\begin{aligned}
\lambda_{f}(w)=\sum_{c \in \sG_f}e_{w:c} \quad \lambda_{m}(w)=\sum_{c \in \sG_m}e_{w:c} \\
\end{aligned}
\label{eq:genderbias:lambda}
\end{equation}

As the values of $\lambda$ appear in a different range than the ones of $\widehat{\lambda}$, to make the approaches comparable, we apply Min-Max normalization on each approach, calculated over the gender factor values of all terms of the corpus. 


%step Since female and male factors in both approaches result in some value between -1 to +1
Another important consideration in our analysis is to distinguish between truly gender-biased terms from low range values of gender factors (which can occur for every random term). To indicate the terms with no considerable inclinations to genders, we define gender-neutrality for a term when the difference between its gender factors is less than a threshold:
\begin{equation}
|\lambda_{f}-\lambda_{m}| < \zeta \quad |\widehat{\lambda}_{f}-\widehat{\lambda}_{m}| < \widehat{\zeta}
\label{eq:genderbias:zeta}
\end{equation}
To find such a threshold for each approach, since the number of gender-specific terms in English are limited, we assume that a randomly sampled term from the vocabulary is a gender-neutral term. This approach is similar to the one used in the Negative Sampling method. We can repeat this sampling for all the terms and calculate the expected values of $\zeta$ and $\widehat{\zeta}$ by averaging $|\lambda_{f}(w)-\lambda_{m}(w)|$ and $|\widehat{\lambda}_{f}(w)-\widehat{\lambda}_{m}(w)|$ respectively over the terms. In our experiments, this results in $\zeta=0.046$ and $\widehat{\zeta}=0.038$.

